Effects of External Radiation Fields on Line Emission - Application to Star-forming Regions

A variety of astronomical environments contain clouds irradiated by a combination of isotropic and beamed radiation fields. For example, molecular clouds may be irradiated by the isotropic cosmic microwave background (CMB), as well as by a nearby active galactic nucleus (AGN). These radiation fields excite atoms and molecules and produce emission in different ways. We revisit the escape probability theorem and derive a novel expression that accounts for the presence of external radiation fields. We show that when the field is isotropic the escape probability is reduced relative to that in the absence of external radiation. This is in agreement with previous results obtained under ad hoc assumptions or with the two-level system, but can be applied to complex many-level models of atoms or molecules. This treatment is in the development version of the spectral synthesis code Cloudy. We examine the spectrum of a Spitzer cloud embedded in the local interstellar radiation field, and show that about 60 percent of its emission lines are sensitive to background subtraction. We argue that this geometric approach could provide an additional tool toward understanding the complex radiation fields of starburst galaxies.

==> macros.tex <==
% some names we use
\newcommand{\Cloudy}{\textsc{Cloudy}}
\newcommand{\Hazy}{\textsc{Hazy}}
\newcommand{\cdCommand}[1]{\textbf{#1}}
\newcommand{\cdVariable}[1]{\emph{#1}}
\newcommand{\cdSectionTitle}[1]{\emph{#1}}
\newcommand{\cdFilename}[1]{\texttt{#1}}
\newcommand{\cdRoutine}[1]{\emph{#1}}
\newcommand{\cdTerm}[1]{\textbf{\emph{#1}}}
\newcommand{\cdMono}[1]{\texttt{#1}}
\newcommand{\fixit}[1]{\textbf{FIXIT: #1}}
\font\manual=manfnt at 7pt \def\dbend{\hbox{\raise0.9ex\hbox{\manual\char127\hspace{0.6em}}}}
\newcommand{\experimental}{\texorpdfstring{\dbend}{??}}

% or symbol provided by Will H
\newcommand\OR{\texorpdfstring{\ensuremath{\vert}}{|}}

% Matt's 1.23\e{-2} 
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}


% \ion from Will, replace AAS version
\newcommand\Ion[2]{\ensuremath{\mathrm{#1\,\scriptstyle #2}}}

% macro sometimes found in ADS bibtex entries
\newcommand{\mdash}{---} 

% ion is in the aas style
\newcounter{INTERNALionstage}
\providecommand{\ion}[2]{% replace the aastex version
  \setcounter{INTERNALionstage}{#2}%
  \Ion{#1}{\Roman{INTERNALionstage}}}

\providecommand{\red}[1]{{\color{red}#1}}

% Will's todo and done macros
%\newcommand\TODO[1]{\textbf{\boldmath [#1]}}
\newcommand{\TODO}[1]{\textcolor{red}{{\textbf{\boldmath [#1]}}}}
\newcommand\DONE[1]{{\color{green!50!gray} \textbf{DONE}} {\color{white!80!black!80!green} #1}}

\newcommand{\Av}{A$_{\rm V}$}

\def\gtsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\Msunpyr{M$_{\odot}\,$yr$^{-1}$}
\def\Msun{M$_{\odot}$}
%       Based on PATs UNITS.TEX with some additions
%
%       Simple units
%
\def\A{{\rm\thinspace \AA}}
\def\cm{{\rm\thinspace cm}}
\def\as{{\rm\thinspace arcsec}}
\def\erg{{\rm\thinspace erg}}
\def\eV{{\rm\thinspace eV}}
\def\g{{\rm\thinspace g}}
\def\ga{{\rm\thinspace gauss}}
\def\hr{{\rm\thinspace hr}}
\def\Hz{{\rm\thinspace Hz}}
\def\K{{\rm\thinspace K}}
\def\keV{{\rm\thinspace keV}}
\def\km{{\rm\thinspace km}}
\def\kpc{{\rm\thinspace kpc}}
\def\Lsun{\mbox{$\rm\thinspace L_{\odot}$}}
\def\m{{\rm\thinspace m}}
\def\MeV{{\rm\thinspace MeV}}
\def\mJy{{\rm\thinspace mJy}}
\def\micron{\hbox{$\mu$m}}
\def\Mpc{{\rm\thinspace Mpc}}
\def\Msun{\mbox{$\rm\thinspace M_{\odot}$}}
\def\nm{{\rm\thinspace nm}}
\def\pc{{\rm\thinspace pc}}
\def\ps{{\rm\thinspace s^{-1}}}
\def\pcc{{\rm\thinspace cm^{-3}}}
\def\Ryd{{\rm\thinspace Ryd}}
\def\s{{\rm\thinspace s}}
\def\sr{{\rm\thinspace sr}}
\def\W{{\rm\thinspace W}}
\def\yr{{\rm\thinspace yr}}
%
%       Compound units
%
\def\keVscm{\mbox{$\keV\cm^{2}\,$}}
\def\cmps{\mbox{$\cm\s^{-1}\,$}}
\def\cmpss{\mbox{$\cm\s^{-2}\,$}}
\def\ergpccmps{\mbox{$\erg\cm^{-3}\s^{-1}\,$}}
\def\ergpg{\mbox{$\erg\g^{-1}\,$}}
\def\ergpscm{\mbox{$\erg\cm^{-2}\,$}}
\def\ergpscmps{\mbox{$\erg\cm^{-2}\s^{-1}\,$}}
\def\ergpscmpspsas{\mbox{$\erg\cm^{-2}\s^{-1}\as^{-2}\,$}}
\def\ergpscmpspa{\mbox{$\erg\cm^{-2}\s^{-1}\A^{-1}\,$}}
\def\ergps{\mbox{$\erg\s^{-1}\,$}}
\def\gpcm{\mbox{$\g\cm^{-3}\,$}}
\def\gpcmps{\mbox{$\g\cm^{-3}\s^{-1}\,$}}
\def\gps{\mbox{$\g\s^{-1}\,$}}
\def\uJy{\mbox{$\mu${\rm Jy}}}
\def\kmps{\mbox{$\km\ps\,$}}
\def\kmpspMpc{\mbox{$\kmps\Mpc^{-1}\,$}}
\def\Lsunppc{\mbox{$\Lsun\pc^{-3}\,$}}
\def\Msunpc{\mbox{$\Msun\pc^{-3}\,$}}
\def\Msunpkpc{\mbox{$\Msun\kpc^{-1}\,$}}
\def\Msunppc{\mbox{$\Msun\pc^{-3}\,$}}
\def\Msunppcpyr{\mbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\def\Msunpyr{\mbox{$\Msun\yr^{-1}\,$}}
\def\Msunpyrpkpc{\mbox{$\Msun\yr^{-1}\kpc^{-1}\,$}}
\def\pscm{\mbox{$\cm^{-2}\,$}}
\def\psm{\mbox{$\m^{-2}\,$}}
\def\pccm{\mbox{$\cm^{-3}\,$}}
\def\pscm{\mbox{$\cm^{-2}\,$}}
\def\pscmps{\mbox{$\cm^{-2}\, \s^{-1}\,$}}
\def\pcm{\mbox{$\m^{-3}\,$}}
\def\pccmK{\mbox{$\cm^{-3}\K$}}
\def\pcmK{\mbox{$\m^{-3}\K$}}
\def\pressure{\mbox{$\g\, \cm^{-1}\, \s^{-2}\,$}}
\def\pyr{\mbox{$\yr^{-1}\,$}}
\def\pyrppc{\mbox{$\yr^{-1}\pc^{-1}\,$}}
\def\scm{\mbox{$\cm^{2}\,$}}
\def\Wpsm{\mbox{$\W\psm\,$}}
\def\Wpscm{\mbox{$\W\pscm\,$}}
\def\WHz{\mbox{$\W\Hz\,$}}
%
% spectral lines
%
\def\la{\mbox{{\rm L}$\alpha$}}
\def\pa{\mbox{{\rm P}$\alpha$}}
\def\ha{\mbox{{\rm H}$\alpha$}}
\def\hb{\mbox{{\rm H}$\beta$}}
\def\hi{\mbox{{\rm H~{\sc i}}}}
\def\hii{\mbox{{\rm H~{\sc ii}}}}
\def\hei{\mbox{{\rm He~{\sc i}}}}
\def\heii{\mbox{{\rm He~{\sc ii}}}}
\def\ci{\mbox{{\rm C~{\sc i}}}}
\def\cii{\mbox{{\rm C~{\sc ii}}}}
\def\ciii{\mbox{{\rm C~{\sc iii}}}}
\def\civ{\mbox{{\rm C~{\sc iv}}}}
\def\ni{\mbox{{\rm N~{\sc i}}}}
\def\nii{\mbox{{\rm N~{\sc ii}}}}
\def\oi{\mbox{{\rm O~{\sc i}}}}
\def\oii{\mbox{{\rm O~{\sc ii}}}}
\def\oiii{\mbox{{\rm O~{\sc iii}}}}
\def\neii{\mbox{{\rm Ne~{\sc ii}}}}
\def\neiii{\mbox{{\rm Ne~{\sc iii}}}}
\def\nev{\mbox{{\rm Ne~{\sc v}}}}
\def\mgii{\mbox{{\rm Mg~{\sc ii}}}}
\def\cliii{\mbox{{\rm Cl~{\sc iii}}}}
\def\sii{\mbox{{\rm S~{\sc ii}}}}
\def\siii{\mbox{{\rm S~{\sc iii}}}}
\def\ariii{\mbox{{\rm Ar~{\sc iii}}}}
\def\caii{\mbox{{\rm Ca~{\sc ii}}}}
\def\fei{\mbox{{\rm Fe~{\sc i}}}}
\def\feii{\mbox{{\rm Fe~{\sc ii}}}}
\def\feiii{\mbox{{\rm Fe~{\sc iii}}}}
\def\feiv{\mbox{{\rm Fe~{\sc iv}}}}
\def\fev{\mbox{{\rm Fe~{\sc v}}}}
\def\fevi{\mbox{{\rm Fe~{\sc vi}}}}
\def\fevii{\mbox{{\rm Fe~{\sc vii}}}}
\def\feviii{\mbox{{\rm Fe~{\sc viii}}}}
\def\feix{\mbox{{\rm Fe~{\sc ix}}}}
\def\fex{\mbox{{\rm Fe~{\sc x}}}}
\def\fexi{\mbox{{\rm Fe~{\sc xi}}}}
\def\fexii{\mbox{{\rm Fe~{\sc xii}}}}
\def\fexiii{\mbox{{\rm Fe~{\sc xiii}}}}
\def\fexiv{\mbox{{\rm Fe~{\sc xiv}}}}
\def\fexv{\mbox{{\rm Fe~{\sc xv}}}}
\def\fexvi{\mbox{{\rm Fe~{\sc xvi}}}}
\def\fexvii{\mbox{{\rm Fe~{\sc xvii}}}}
\def\fexviii{\mbox{{\rm Fe~{\sc xviii}}}}
\def\fexix{\mbox{{\rm Fe~{\sc xix}}}}
\def\fexx{\mbox{{\rm Fe~{\sc xx}}}}
\def\fexxi{\mbox{{\rm Fe~{\sc xxi}}}}
\def\fexxii{\mbox{{\rm Fe~{\sc xxii}}}}
\def\fexxiii{\mbox{{\rm Fe~{\sc xxiii}}}}
\def\fexxiv{\mbox{{\rm Fe~{\sc xxiv}}}}
\def\fexxv{\mbox{{\rm Fe~{\sc xxv}}}}
\def\fexxvi{\mbox{{\rm Fe~{\sc xxvi}}}}
%
% types of baryons
\def\water{\mbox{{\rm H}$_2${\rm O}}}
\def\CO{\mbox{{\rm CO}}}
\def\OH{\mbox{{\rm OH}}}
\def\htwo{\mbox{{\rm H}$_2$}}
\def\hone{\mbox{{\rm H}$^0$}}
\def\hplus{\mbox{{\rm H}$^+$}}
\def\hminus{\mbox{{\rm H}$^-$}}
% cannot have numbers in names, so cap Oh represents zero
\def\hO{\mbox{{\rm H}$^0$}}
\def\heO{\mbox{{\rm He}$^0$}}
\def\heo{\mbox{{\rm He}$^0$}}
\def\heplus{\mbox{{\rm He}$^+$}}
\def\hePP{\mbox{{\rm He}$^{2+}$}}
\def\cO{\mbox{{\rm C}$^0$}}
\def\cplus{\mbox{{\rm C}$^+$}}
%
\def\Hrec{\mbox{${\rm H}_{rec}$}}
%\def\Hrec{\mbox{$H_{rec}$}}
\def\centreline{\centerline}
%
% Nina
\DeclareMathAlphabet{\vib}{OML}{cmm}{m}{it}
% From Glenn
\newcommand*{\satellite}[1]{\textit{#1}}
\newcommand*{\xmm}{\satellite{XMM-Newton}}
\newcommand*{\chandra}{\satellite{Chandra}}
\newcommand*{\asca}{\satellite{ASCA}}
\newcommand*{\rosat}{\satellite{ROSAT}}
\newcommand*{\prog}[1]{\textsc{#1}}
%% For kb, mH. etc. Italic with non-italic subscript.
\newcommand*{\mysub}[2]{\ensuremath{#1_{\mathrm{#2}}}}

